DEFOM-Stereo: Depth Foundation Model Based Stereo Matching

Stereo matching is a key technique for metric depth estimation in computer vision and robotics. Real-world challenges like occlusion and non-texture hinder accurate disparity estimation from binocular matching cues. Recently, monocular relative depth estimation has shown remarkable generalization using vision foundation models. Thus, to facilitate robust stereo matching with monocular depth cues, we incorporate a robust monocular relative depth model into the recurrent stereo-matching framework, building a new framework for depth foundation model-based stereo-matching, DEFOM-Stereo. In the feature extraction stage, we construct the combined context and matching feature encoder by integrating features from conventional CNNs and DEFOM. In the update stage, we use the depth predicted by DEFOM to initialize the recurrent disparity and introduce a scale update module to refine the disparity at the correct scale. DEFOM-Stereo is verified to have much stronger zero-shot generalization compared with SOTA methods. Moreover, DEFOM-Stereo achieves top performance on the KITTI 2012, KITTI 2015, Middlebury, and ETH3D benchmarks, ranking $1^{st}$ on many metrics. In the joint evaluation under the robust vision challenge, our model simultaneously outperforms previous models on the individual benchmarks, further demonstrating its outstanding capabilities.

==> figs/scale_inc.tex <==
\begin{subfigure}{1.0\linewidth}
    \begin{subfigure}{0.323\linewidth}
        \centering
        \begin{overpic}[width=1.0\linewidth]{figs/main/A_0104_0013_left.jpg}
            \put(1, 2){\textcolor{white}{\footnotesize{Left Image}}}
        \end{overpic}
    \end{subfigure}
    \begin{subfigure}{0.323\linewidth}
        \centering
        \begin{overpic}[width=1.0\linewidth]{figs/main/A_0104_0013_danv2.jpg}
            \put(1, 2){\textcolor{white}{\footnotesize{Depth Anything V2}}}
        \end{overpic}
    \end{subfigure}
    \begin{subfigure}{0.323\linewidth}
        \centering
        \begin{overpic}[width=1.0\linewidth]{figs/main/A_0104_0013_gt.jpg}
            \put(0, 2){\textcolor{white}{\footnotesize{Ground-Truth Disparity}}}
        \end{overpic}
    \end{subfigure}
    \vspace{-7pt}
\end{subfigure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

